Interpreting and Exploiting Functional Specialization in Multi-Head Attention under Multi-task Learning

Transformer-based models, even though achieving super-human performance on several downstream tasks, are often regarded as a black box and used as a whole. It is still unclear what mechanisms they have learned, especially their core module: multi-head attention. Inspired by functional specialization in the human brain, which helps to efficiently handle multiple tasks, this work attempts to figure out whether the multi-head attention module will evolve similar function separation under multi-tasking training. If it is, can this mechanism further improve the model performance? To investigate these questions, we introduce an interpreting method to quantify the degree of functional specialization in multi-head attention. We further propose a simple multi-task training method to increase functional specialization and mitigate negative information transfer in multi-task learning. Experimental results on seven pre-trained transformer models have demonstrated that multi-head attention does evolve functional specialization phenomenon after multi-task training which is affected by the similarity of tasks. Moreover, the multi-task training strategy based on functional specialization boosts performance in both multi-task learning and transfer learning without adding any parameters.

==> tabs/InterpretingImportantHeads.tex <==
\begin{table*}[htp]

\renewcommand\arraystretch{1.2}

\centering
\small
\vspace{-0.4cm}

\setlength{\tabcolsep}{1.2mm}
 \begin{tabu}{ccccccccccc}
 
 \toprule[1.2pt]
  & \multicolumn{2}{c}{\textbf{Surface}} & \multicolumn{3}{c}{\textbf{Syntactic}} &    \multicolumn{5}{c}{\textbf{Semantic}} \\
  \cmidrule(r){2-3}  \cmidrule(r){4-6} \cmidrule(r){7-11} \noalign{\smallskip}
\multicolumn{1}{c}{\textbf{Task}}& \textbf{\scriptsize Length}&\textbf{\scriptsize WordContent}& \textbf{\scriptsize Depth}&\textbf{\scriptsize TopConst}& \textbf{\scriptsize BigramShift}&\textbf{\scriptsize Tense} & \textbf{\scriptsize SubjNum}&\textbf{\scriptsize ObjNum}& \textbf{\scriptsize OddManOut}& \textbf{\scriptsize CoordInversion}\\
   \midrule[0.8pt]
 Head Avg.    & $50.89$ & $10.60$ & $22.61$  &  $34.44$ & $57.46$ &  $69.96$ & $64.16$ & $63.59$ & $51.93$ & $53.26$ \\ 
 \specialrule{0em}{0pt}{0pt}

 MNLI    & $56.98$            & $8.91$  & $24.00$               &  $37.95$ & $\textbf{58.54}$ &  $71.28$ & $66.95$ & $\textbf{66.33}$ & $51.88$ & $53.02$ \\ 
 \specialrule{0em}{0pt}{0pt}

 QQP    & $60.82$             & $9.86$  & $24.42$               &  $37.64$ & $58.14$           &  $\textbf{71.75}$ & $66.63$ & $66.21$ & $51.88$ & $52.58$ \\ 
 \specialrule{0em}{0pt}{0pt}

 QNLI   & $\underline{56.95}$ & $9.71$  & $\underline{23.97}$   &  $37.59$ & $\textbf{58.54}$ &  $71.69$ & $\textbf{67.11}$ & $66.30$ & $\textbf{51.99}$ & $\textbf{53.19}$ \\ 
 \specialrule{0em}{0pt}{0pt}

 AG   & $\textbf{64.58}$      & $\textbf{10.01}$ & $\textbf{24.94}$  &  $\underline{37.31}$ & $\underline{56.62}$ &  $71.67$ & $\underline{66.12}$ & $\underline{65.97}$ & $\underline{51.59}$ & $\underline{52.15}$ \\ 
 \specialrule{0em}{0pt}{0pt}
  
 SST-2   & $60.13$             & $\underline{8.78}$ & $24.45$   &  $\textbf{38.01}$ & $57.64$ &  $\underline{70.76}$ & $66.57$ & $66.09$ & $51.70$ & $52.65$ \\ 
 \specialrule{0em}{0pt}{0pt}
\bottomrule[1.2pt]
\end{tabu}
\caption{\label{tab:probing_performance} Average performance of top-30\% important attention heads for each task on ten probing tasks. The first row is the average performance of all attention heads in $\text{BERT}_{\text{BASE}}$ on probing tasks. 
}
\vspace{-5mm}

\end{table*}

==> tabs/algorithm.tex <==
\begin{algorithm}[htb] 
\small

\caption{Important Attention-head Training} 
\label{alg:generate}
\begin{algorithmic}[1] %这个1 表示每一行都显示数字

\REQUIRE ~~\\
$X^{(i)} = \left\{ x_{1}^{i},x_{2}^{i},\ldots,x_{n_i}^{i} \right\}$, training samples of task $i$;\\
$\delta$, proportion of important attention-head training;\\
$\lambda$, proportion of top important attention heads to train;\\
$f$, a multitask model;\\
$S$, total training steps;
\ENSURE ~~\\
$\widehat{X} = \left\{ \hat{x}_{1},\hat{x}_{2},\ldots,\hat{x}_{n} \right\}$, adversarial example;
\STATE $\left. \widehat{X}\gets X \right.$
\IF{$f\left( X \right) \neq Y$}
  \RETURN $\widehat{X}$
\ELSE
  \STATE $\left. num\leftarrow 0 \right.$
  \WHILE{$f(\widehat{X}) = Y\ \&\&\ num \leq \lambda \cdot n$ }
    \STATE $O=\{o_1,o_2,...,o_n\} \gets $ Logit output of $f(\widehat{X})$ \
    \STATE $P=\{p_1,p_2,...,p_k\} \gets$ Sort the position $p_i$ in ascending order based on $s_{p_i}\ (\ 1\le p_i\le n$ and $y_{p_i} $ is a Chinese character\ )\
    \FOR{each $i \in [1,k]$}
      \IF{$\hat{x}_{p_{i}} \neq y_{p_{i}}$}
        \STATE {\bf continue}
      \ENDIF
    \STATE $\left. \hat{x}_{p_{i}}\gets m_{p_{i}} \right.$, where $m_{p_{i}} \in D\left( x_{p_{i}} \right)$ and $p_{i}^{m_{p_{i}}} = max\left\{ p_{i}^{r},p_{i}^{r} \in D\left( x_{p_{i}} \right) \right\}$
    \STATE {\bf break}
    \ENDFOR
  \STATE $\left. num\gets num + 1 \right.$
  \ENDWHILE
\ENDIF
\RETURN $\widehat{X}$
\end{algorithmic}

\end{algorithm}

==> tabs/dual_task/bert_base.tex <==
\setlength{\tabcolsep}{1.7mm}
\begin{table}[h]
	\centering
	\small
	\renewcommand\arraystretch{1.3}
	% \vspace{-0.4cm}
	\begin{center}
		\begin{tabular}{cccccc}
			\toprule[1.2pt]
			\textbf{Task}                   & $\text{MNLI}_A$   & $\text{QQP}_A$    & $\text{QNLI}_A$ 	& $\text{AG}_A$     & $\text{SST-2}_A$ 	\\
			\midrule[0.8pt]
			$\text{MNLI}_B$                 & -  		        & 2.601  	        & 2.631 	        & \textbf{16.262}	& 0.206  	        \\
			$\text{QQP}_B$                  & 2.780	            & - 		        & 4.823 	        & 10.387	        & 3.183 	        \\
			$\text{QNLI}_B$                 & 2.337	            & 1.922 	        & - 		        & 6.905	            & 3.282  	        \\
			$\text{AG}_B$                   & 11.364	        & \textbf{28.969} 	& 13.270 	        & - 		        & \textbf{4.051} 	\\
			$\text{SST-2}_B$                & \textbf{13.812}   & 11.340 	        & \textbf{32.871}   & 2.982	            & -        	        \\
			\bottomrule[1.2pt]
		\end{tabular}
		\caption{Dissociation score of task A in dual-task learning tasks with $\theta=30\%$ using $\text{BERT}_{\text{BASE}}$. "$\text{Task}_A$" denotes the task A of dual-task learning.
  % 加一个平均得分计算
  }
		\label{tab:2tasksBertBase}
	\end{center}
	% \vspace{-5mm}
\end{table}

==> tabs/dual_task/bert_baseline.tex <==
\setlength{\tabcolsep}{1.7mm}
\begin{table}[h]
	\centering
	\small
	\renewcommand\arraystretch{1.3}
	% \vspace{-0.4cm}
	\begin{center}
		\begin{tabular}{cccccc}
			\toprule[1.2pt]
			\textbf{Task}                   & $\text{MNLI}_A$   & $\text{QQP}_A$    & $\text{QNLI}_A$ 	& $\text{AG}_A$     & $\text{SST-2}_A$ 	\\
			\midrule[0.8pt]
			$\text{MNLI}_B$                 & -  		        & 0.354  	        & 1.208 	        & \textbf{4.528}	& 1.203  	        \\
			$\text{QQP}_B$                  & -0.963	        & - 		        & 0.151 	        & 3.936	            & \textbf{6.952} 	\\
			$\text{QNLI}_B$                 & -0.132	        & 0.007 	        & - 		        & 0.903	            & 2.139  	        \\
			$\text{AG}_B$                   & \textbf{5.589}	& \textbf{0.820} 	& 6.744 	        & - 		        & 3.898 	        \\
			$\text{SST-2}_B$                & 3.267             & -1.072 	        & \textbf{7.675}    & 2.475	            & -        	        \\
			\bottomrule[1.2pt]
		\end{tabular}
		\caption{Summary of $D_A(\theta)$ in dual-task learning tasks with $\theta=30\%$ using a \textbf{frozen} $\text{BERT}_{\text{BASE}}$ encoder.}
		\label{tab:2tasksBertBaseline}
	\end{center}
	\vspace{-5mm}
\end{table}

==> tabs/dual_task/bert_large.tex <==
\setlength{\tabcolsep}{1.7mm}
\begin{table}[h]
	\centering
	\small
	\renewcommand\arraystretch{1.3}
	% \vspace{-0.4cm}
	\begin{center}
		\begin{tabular}{cccccc}
			\toprule[1.2pt]
			\textbf{Task}                   & $\text{MNLI}_A$   & $\text{QQP}_A$    & $\text{QNLI}_A$ 	& $\text{AG}_A$     & $\text{SST-2}_A$ 	\\
			\midrule[0.8pt]
			$\text{MNLI}_B$                 & -  		        & 0.826  	        & 3.554 	        & 6.157	            & \textbf{9.808}  	\\
			$\text{QQP}_B$                  & 2.429	            & - 		        & 5.898 	        & 2.882	            & 6.522 	        \\
			$\text{QNLI}_B$                 & 5.689	            & 0.022 	        & - 		        & \textbf{9.559}	& 8.735  	        \\
			$\text{AG}_B$                   & 17.308	        & \textbf{22.403} 	& 17.905 	        & - 		        & 7.234 	        \\
			$\text{SST-2}_B$                & \textbf{19.829}   & 21.197 	        & \textbf{20.444}   & 7.717	            & -        	        \\
			\bottomrule[1.2pt]
		\end{tabular}
		\caption{Summary of $D_A(\theta)$ in dual-task learning tasks with $\theta=30\%$ using $\text{BERT}_{\text{LARGE}}$. "$\text{Task}_A$" denotes the task A of dual-task learning.}
		\label{tab:2tasksBertLarge}
	\end{center}
	% \vspace{-5mm}
\end{table}

==> tabs/dual_task/bert_tiny.tex <==
\setlength{\tabcolsep}{1.7mm}
\begin{table}[h]
	\centering
	\small
	\renewcommand\arraystretch{1.3}
	% \vspace{-0.4cm}
	\begin{center}
		\begin{tabular}{cccccc}
			\toprule[1.2pt]
			\textbf{Task}                   & $\text{MNLI}_A$   & $\text{QQP}_A$    & $\text{QNLI}_A$ 	& $\text{AG}_A$     & $\text{SST-2}_A$ 	\\
			\midrule[0.8pt]
			$\text{MNLI}_B$                 & -  		        & 20.101  	        & 1.194 	        & 5.363	            & \textbf{4.714}  	\\
			$\text{QQP}_B$                  & 2.042	            & - 		        & 0.629 	        & \textbf{6.538}	& 2.345 	        \\
			$\text{QNLI}_B$                 & 3.818	            & 14.420 	        & - 		        & 6.282	            & 1.633  	        \\
			$\text{AG}_B$                   & \textbf{35.657}	& 8.696 	        & 14.870 	        & - 		        & 1.592 	        \\
			$\text{SST-2}_B$                & 31.848            & \textbf{24.395} 	& \textbf{35.590}   & 1.077	            & -        	        \\
			\bottomrule[1.2pt]
		\end{tabular}
		\caption{Summary of $D_A(\theta)$ in dual-task learning tasks with $\theta=30\%$ using TinyBERT-6L."$\text{Task}_A$" denotes the task A of dual-task learning.}
		\label{tab:2tasksBertTiny}
	\end{center}
	% \vspace{-5mm}
\end{table}

==> tabs/dual_task/debertaV3.tex <==
\setlength{\tabcolsep}{1.7mm}
\begin{table}[h]
	\centering
	\small
	\renewcommand\arraystretch{1.3}
	% \vspace{-0.4cm}
	\begin{center}
		\begin{tabular}{cccccc}
			\toprule[1.2pt]
			\textbf{Task}                   & $\text{MNLI}_A$   & $\text{QQP}_A$    & $\text{QNLI}_A$ 	& $\text{AG}_A$     & $\text{SST-2}_A$ 	\\
			\midrule[0.8pt]
			$\text{MNLI}_B$                 & -  		        & 4.640  	        & 0.019 	        & 8.466	            & 2.645  	        \\
			$\text{QQP}_B$                  & 6.212	            & - 		        & 0.020 	        & 9.501	            & 13.333 	        \\
			$\text{QNLI}_B$                 & 14.210	        & 9.503 	        & - 		        & \textbf{16.919}	& 2.327  	        \\
			$\text{AG}_B$                   & 24.107	        & 11.648 	        & 3.422 	        & - 		        & \textbf{17.778} 	\\
			$\text{SST-2}_B$                & \textbf{27.032}   & \textbf{20.506} 	& \textbf{20.360}   & 4.972	            & -        	        \\
			\bottomrule[1.2pt]
		\end{tabular}
		\caption{Summary of $D_A(\theta)$ in dual-task learning tasks with $\theta=30\%$ using $\text{DeBERTaV3}_{\text{BASE}}$. "$\text{Task}_A$" denotes the task A of dual-task learning.}
		\label{tab:2tasksDebertaV3}
	\end{center}
	\vspace{-5mm}
\end{table}

==> tabs/dual_task/roberta_base.tex <==
\setlength{\tabcolsep}{1.7mm}
\begin{table}[h]
	\centering
	\small
	\renewcommand\arraystretch{1.3}
	% \vspace{-0.4cm}
	\begin{center}
		\begin{tabular}{cccccc}
			\toprule[1.2pt]
			\textbf{Task}                   & $\text{MNLI}_A$   & $\text{QQP}_A$    & $\text{QNLI}_A$ 	& $\text{AG}_A$     & $\text{SST-2}_A$ 	\\
			\midrule[0.8pt]
			$\text{MNLI}_B$                 & -  		        & 10.858            & 4.317             & 38.226            & \textbf{8.398}  	\\
			$\text{QQP}_B$                  & 8.556             & - 		        & 0.537 	        & 22.726	        & 5.591             \\
			$\text{QNLI}_B$                 & 1.307	            & 2.430 	        & - 		        & \textbf{47.728}   & 5.012  	        \\
			$\text{AG}_B$                   & \textbf{17.430}   & \textbf{23.268} 	& 15.962 	        & - 		        & 6.157             \\
			$\text{SST-2}_B$                & 5.481             & 22.186 	        & \textbf{16.092}   & 6.619	            & -        	        \\
			\bottomrule[1.2pt]
		\end{tabular}
	\end{center}
	\caption{Summary of $D_A(\theta)$ in dual-task learning tasks with $\theta=30\%$ using $\text{RoBERTa}_{\text{BASE}}$. "$\text{Task}_A$" denotes the task A of dual-task learning.}
	\label{tab:2tasksRoberta}
% 	\vspace{-4mm}
\end{table}

==> tabs/probingTasks.tex <==
\setlength{\tabcolsep}{1.1mm}
\begin{table*}[htp]
	\centering

	\footnotesize
	%\vspace{-0.4cm}
	\renewcommand\arraystretch{1.1}
	\begin{center}
		\begin{tabular}{lccccl}
			\toprule[1.2pt]  
			Task           & \#Train  &\#Test   & \#Class &  Type  & Description \\
			\midrule[0.8pt]
			Length         & 100,000 & 10,000   & 6     &   Surface    & Predict input sentence length \\
                WordContent    & 100,000 & 10,000   & 1000  &   Surface	    & Predict which word is contained in sentence \\
			\midrule[0.8pt]
                Depth          & 100,000 & 10,000   & 8 	 &   Syntactic   & Predict maximum depth of syntactic tree \\
                TopConst       & 100,000 & 10,000   & 20     &   Syntactic	    & Predict top-constituent  \\
			BigramShift    & 100,000 & 10,000   & 2 	 &   Syntactic   & Detect bigram order perturbation \\
                \midrule[0.8pt]
			Tense          & 100,000 & 10,000   & 2 	&   Semantic    & Predict the tense of main verb  \\
			SubjNum        & 100,000 & 10,000   & 2 	&   Semantic    & Predict whether a subject is plural \\
                ObjNum         & 100,000 & 10,000   & 2     &   Semantic    & Predict whether an object is plural \\
                OddManOut      & 100,000 & 10,000   & 2     &   Semantic    & Detect noun or verb perturbation \\
                CoordInversion & 100,000 & 10,000   & 2     &   Semantic    & Detect clausal order perturbation \\
			\bottomrule[1.2pt]
		\end{tabular}
		\caption{Summary of sentence probing tasks in SentEval toolkit.}
		\label{tab:probingTasks}
	\end{center}
	\vspace{-5mm}
\end{table*}

==> tabs/transfer_scitail.tex <==
\begin{table}[tp]

\renewcommand\arraystretch{1.2}

\centering
\small

\setlength{\tabcolsep}{0.8mm}
 \begin{tabu}{lcccc}
 
 \toprule[1.2pt]
   &  \multicolumn{4}{c}{\textbf{\% data of SciTail}} \\
  \cmidrule(r){2-5}  \noalign{\smallskip}
\multicolumn{1}{c}{\textbf{Model}} & \textbf{0.1\%}&\textbf{1\%}& \textbf{10\%}&\textbf{100\%}\\

   \midrule[0.8pt]
 % $\text{BERT}_{\text{BASE}}^{1}$     & $51.2$    & $82.2$      & $90.5$          & $94.3$  \\ 

 $\text{MT-DNN}^{1}$                 & $81.9$    & $88.3$      & $91.1$         & $95.7$   \\ 
 
 $\text{MT-DNN}_{\text{SMART}}^{2}$  & $82.3$    & $88.6$      & $91.3$          & $96.1$ \\ 
 
 $\text{CA-MTL}_{\text{BASE}}^{3}$   & $83.2$    & $88.7$      & $91.4$         & $95.6$ \\

 $\text{Ticket-Share}_{\text{BASE}}^{4}$   & $83.1$    & $\textbf{90.1}$      & $\textbf{93.5}$         & $\textbf{96.5}$ \\
  %\midrule[0.8pt]
  \cdashlinelr{1-5}
  
 $\text{BERT}_{\text{BASE}}$ & $82.0_{\pm 7.6}$       & $88.1_{\pm 1.3}$      & $91.9_{\pm 0.7}$          & $95.5_{\pm 0.2}$  \\ 
 \specialrule{0em}{0pt}{0pt}

 \ \ \ \ \ \ \ \ +IAT                    & $\textbf{83.3}_{\pm 6.7}$       & $89.2^*_{\pm 1.0}$      & $92.5^*_{\pm 0.5}$          & $\text{95.9}^*_{\pm 0.1}$    \\  
 \specialrule{0em}{0pt}{0pt}
 
\bottomrule[1.2pt]

\end{tabu}
\caption{\label{tab:transfer_dev} Transfer learning results on development sets (${}^{*}$ indicates statistically significant improvements at the $5\%$ level). All models use $\text{BERT}_{\text{BASE}}$ as encoder and are initialized from their multi-task learning models on GLUE. Results from: \citet{liu-etal-2019-multi}${}^1$, \citet{jiang-etal-2020-smart}${}^2$, \citet{pilault2021conditionally}${}^3$, \citet{liang-etal-2021-super}${}^4$.
}
\end{table}
